MaIL: Improving Imitation Learning with Mamba

This work presents Mamba Imitation Learning (MaIL), a novel imitation learning (IL) architecture that provides an alternative to state-of-the-art (SoTA) Transformer-based policies. MaIL leverages Mamba, a state-space model designed to selectively focus on key features of the data. While Transformers are highly effective in data-rich environments due to their dense attention mechanisms, they can struggle with smaller datasets, often leading to overfitting or suboptimal representation learning. In contrast, Mamba's architecture enhances representation learning efficiency by focusing on key features and reducing model complexity. This approach mitigates overfitting and enhances generalization, even when working with limited data. Extensive evaluations on the LIBERO benchmark demonstrate that MaIL consistently outperforms Transformers on all LIBERO tasks with limited data and matches their performance when the full dataset is available. Additionally, MaIL's effectiveness is validated through its superior performance in three real robot experiments. Our code is available at https://github.com/ALRhub/MaIL.

==> figures/method_illustration/method_fig.tex <==
% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/method_illustration/fig/method.png}
%     \caption{\todo{TBD}}
%     \label{fig:method_illustration}
% \end{figure}

==> results/tables/d3il.tex <==
\begin{table}[!t]
    \centering
    % \tiny
    % \scriptsize
    \footnotesize
    \setlength{\aboverulesep}{0pt}
    \setlength{\belowrulesep}{0pt}
    \renewcommand{\arraystretch}{1.}    
    \tiny
    \begin{subtable}[t]{1.0\linewidth}
        \centering
        \input{results/tables/d3il_success}
        \caption{Task Success Rate}
        \label{tab:distill_success}
    \end{subtable}
    \\
    \begin{subtable}[t]{1.0\linewidth}
        \centering
        \input{results/tables/d3il_entropy}
        \caption{Task Entropy}
        \label{tab:distill_entropy}
    \end{subtable}
    \vspace{-0.15cm}
    \caption{Comparison on the D3IL benchmark. The baseline results are from the D3IL paper and all methods are tested across 6 seeds.}
    \label{tab:d3il_results}
    \renewcommand{\arraystretch}{1}
    \vspace{-0.25cm}
\end{table}

==> results/tables/d3il_entropy.tex <==
% \begin{table}[hbtp]
% \centering
% \caption{History ablation on LIBERO}\label{main_results}
 
% \resizebox{.9\textwidth}{!}{  

\begin{tabular}{l|cccccc}
	\toprule 

          & \textbf{Avoiding} & \textbf{Aligning} & \textbf{Pushing} & \textbf{Sorting-4} & \textbf{Sorting-4 (image)} & \textbf{Stacking (image)}  \\

        \midrule
        
        \textbf{DDPM-GPT}  & $0.898 \scriptstyle{\pm 0.018}$ & $0.664 \scriptstyle{\pm 0.075}$ & $0.862 \scriptstyle{\pm 0.017}$ & $0.372 \scriptstyle{\pm 0.068}$ 
        \\
        
        \textbf{BESO}  & $0.856 \scriptstyle{\pm 0.018}$ & $0.711 \scriptstyle{\pm 0.030}$ & $0.871 \scriptstyle{\pm 0.037}$ & $0.232 \scriptstyle{\pm 0.040}$ 
        \\
        \textbf{DDPM-ACT}  & $0.863 \scriptstyle{\pm 0.068}$ & $0.749 \scriptstyle{\pm 0.041}$ & $0.859 \scriptstyle{\pm 0.012}$ & $0.300 \scriptstyle{\pm 0.051}$ 
        \\

        \midrule
        
        \textbf{DDPM-Mamba} & $0 \scriptstyle{\pm 0}$ & $0.694 \scriptstyle{\pm 0.080}$ 
        \\
        \textbf{DDPM-MambaCross} & $0 \scriptstyle{\pm 0}$ & $\mathbf{0.774 \scriptstyle{\pm 0.058}}$
        \\
        
	\midrule
        
\end{tabular}

% }
% \vskip -0.15in
% \end{table}

==> results/tables/d3il_success.tex <==
% \begin{table}[hbtp]
% \centering
% \caption{History ablation on LIBERO}\label{main_results}
 
% \resizebox{.9\textwidth}{!}{  

\begin{tabular}{l|cccccc}
	\toprule 

          & \textbf{Avoiding} & \textbf{Aligning} & \textbf{Pushing} & \textbf{Sorting-4} & \textbf{Sorting-4 (image)} & \textbf{Stacking (image)}  \\

        \midrule
        
        \textbf{DDPM-GPT}  & $0.927 \scriptstyle{\pm 0.022}$ & $0.839 \scriptstyle{\pm 0.020}$ & $0.847 \scriptstyle{\pm 0.862}$ & $0.337 \scriptstyle{\pm 0.084}$
        \\
        
        \textbf{BESO}  & $0.950 \scriptstyle{\pm 0.015}$ & $0.861 \scriptstyle{\pm 0.016}$ & $0.794 \scriptstyle{\pm 0.095}$ & $0.188 \scriptstyle{\pm 0.042}$
        \\
        \textbf{DDPM-ACT}  & $0.899 \scriptstyle{\pm 0.006}$ & $0.849 \scriptstyle{\pm 0.023}$ & $0.920 \scriptstyle{\pm 0.027}$ & $0.300 \scriptstyle{\pm 0.060}$
        \\

        \midrule
        
        \textbf{DDPM-Mamba} & $0 \scriptstyle{\pm 0}$ & $\mathbf{0.884 \scriptstyle{\pm 0.018}}$ 
        \\
        \textbf{DDPM-MambaCross} & $0 \scriptstyle{\pm 0}$ & $0.875 \scriptstyle{\pm 0.014}$
        \\
        
	\midrule
        
\end{tabular}

% }
% \vskip -0.15in
% \end{table}

==> results/tables/data_aug.tex <==
\begin{table}[hbtp]
\centering
\caption{Data augmentation ablation on LIBERO}\label{data_aug}
 
\resizebox{.95\textwidth}{!}{  

\begin{tabular}{l|cc|cc|cc}
	\toprule 

         history=5 & \multicolumn{2}{c|}{aug\_factor=0.1} & \multicolumn{2}{c|}{aug\_factor=0.2} & \multicolumn{2}{c}{aug\_factor=0.3}  \\

        \midrule
                & Libero-Object & Libero-Spatial & Libero-Object & Libero-Spatial & Libero-Object & Libero-Spatial \\
        
        DDPM-Dec  & $0.745 \scriptstyle{\pm 0.118}$ & $0.365 \scriptstyle{\pm 0.048}$ & $0.708 \scriptstyle{\pm 0.071}$ & $0.367 \scriptstyle{\pm 0.038}$ & $0.658 \scriptstyle{\pm 0.089}$ & $0.357 \scriptstyle{\pm 0.063}$
        \\
        DDPM-EncDec  & $0.687 \scriptstyle{\pm 0.040}$ & $0.350 \scriptstyle{\pm 0.078}$ & $0.705 \scriptstyle{\pm 0.096}$ & $0.388 \scriptstyle{\pm 0.073}$
        & $0. \scriptstyle{\pm 0.0}$ & $0.348 \scriptstyle{\pm 0.084}$
        \\
        
        DDPM-Mamba  & $0.782 \scriptstyle{\pm 0.037}$ & $0.467 \scriptstyle{\pm 0.006}$ & $0.780 \scriptstyle{\pm 0.020}$ & $0.485 \scriptstyle{\pm 0.078}$ & $0.617 \scriptstyle{\pm 0.075}$ & $0.452 \scriptstyle{\pm 0.056}$
        \\
        DDPM-MambaDec  & $0.778 \scriptstyle{\pm 0.039}$ & $0.417 \scriptstyle{\pm 0.033}$ & $0.743 \scriptstyle{\pm 0.121}$ & $0.437 \scriptstyle{\pm 0.113}$
        & $0.650 \scriptstyle{\pm 0.0}$ & $0.398 \scriptstyle{\pm 0.132}$
        \\
        
	\midrule
        
\end{tabular}

}
\vskip -0.15in
\end{table}

==> results/tables/history.tex <==
\begin{table}[hbtp]
\centering
\caption{History ablation on LIBERO}\label{main_results}
 
\resizebox{.9\textwidth}{!}{  

\begin{tabular}{l|c|c}
	\toprule 

         history=5 & Libero-Spatial & Libero-Long  \\

        \midrule
        
        DDPM-Dec  & $0.436 \scriptstyle{\pm 0.045}$ & $0.202 \scriptstyle{\pm 0.085}$ 
        \\
        DDPM-EncDec  & $0.382 \scriptstyle{\pm 0.085}$ & $0.296 \scriptstyle{\pm 0.027}$ 
        \\
        
        DDPM-Mamba  & $0.496 \scriptstyle{\pm 0.036}$ & $0.235 \scriptstyle{\pm 0.063}$ 
        \\
        DDPM-MambaDec  & $0.501 \scriptstyle{\pm 0.072}$ & $0.244 \scriptstyle{\pm 0.057}$ 
        \\
        
	\midrule
        
\end{tabular}

}
\vskip -0.15in
\end{table}

==> results/tables/language.tex <==
\begin{table}[hbtp]
\centering
\caption{Language test}\label{main_results}
 
\resizebox{.9\textwidth}{!}{  

\begin{tabular}{l|c|c|c}
	\toprule 

         history=1 & Libero-Goal & Libero-Spatial & Libero-Long \\

        \midrule
        
        DDPM-Dec  & $0 \scriptstyle{\pm 0}$ & $0 \scriptstyle{\pm 0}$ &
        \\
        DDPM-EncDec  & $0 \scriptstyle{\pm 0}$ & $0 \scriptstyle{\pm 0}$ &
        \\
        
        DDPM-Mamba  & $0 \scriptstyle{\pm 0}$ & $0 \scriptstyle{\pm 0}$ &
        \\
        DDPM-MambaDec  & $0 \scriptstyle{\pm 0}$ & $0 \scriptstyle{\pm 0}$ &
        \\
        
	\midrule
        
\end{tabular}

}
\vskip -0.15in
\end{table}

==> results/tables/main_results.tex <==
\begin{table}[hbtp]
\centering
\caption{Average Performance on LIBERO benchmark, where "w/o language" indicates that we do not use language instructions and "w/ language" means we use language tokens generated from a pre-trained CLIP model.}\label{main_results_h1}
 
\resizebox{.95\textwidth}{!}{  

\begin{tabular}{l|c|ccc|cc}
	\toprule 

        & & \multicolumn{3}{c|}{w/o language} & \multicolumn{2}{c}{w/ language}\\
        
         \midrule
         Policy & Backbone & Libero-Object & Libero-Spatial & Libero-Long & Libero-Goal & Libero-90 \\

	\midrule

        BC & D-T  & $0.358 \scriptstyle{\pm 0.086}$ & $0.257 \scriptstyle{\pm 0.030}$ & $0.222 \scriptstyle{\pm 0.067}$ & $0.362 \scriptstyle{\pm 0.034}$ & $0.311 \scriptstyle{\pm 0.055}$
        \\
        & ED-T  & $0.480 \scriptstyle{\pm 0.027}$ & $0.333 \scriptstyle{\pm 0.029}$ & $0.265 \scriptstyle{\pm 0.015}$ & $0.325 \scriptstyle{\pm 0.020}$ & $0.268 \scriptstyle{\pm 0.050}$
        \\
        & D-M  & $0.550 \scriptstyle{\pm 0.062}$ & $\mathbf{0.410 \scriptstyle{\pm 0.058}}$ & $\mathbf{0.287 \scriptstyle{\pm 0.037}}$ & $\mathbf{0.482 \scriptstyle{\pm 0.066}}$ & $\mathbf{0.559 \scriptstyle{\pm 0.021}}$
        \\
        & ED-M  & $\mathbf{0.618 \scriptstyle{\pm 0.058}}$ & $0.352 \scriptstyle{\pm 0.069}$ & $0.275 \scriptstyle{\pm 0.023}$ & $0.473 \scriptstyle{\pm 0.031}$ & $0.514 \scriptstyle{\pm 0.008}$
        \\

        \midrule
        
        DDP & D-T  & $0.667 \scriptstyle{\pm 0.058}$ & $0.473 \scriptstyle{\pm 0.040}$ &
        $0.330 \scriptstyle{\pm 0.029}$ & $0.300 \scriptstyle{\pm 0.350}$ & $0.181 \scriptstyle{\pm 0.024}$ \\
        
        & ED-T  & $0.680 \scriptstyle{\pm 0.027}$ & $0.420 \scriptstyle{\pm 0.022}$ &
        $0.373 \scriptstyle{\pm 0.042}$ & $0.478 \scriptstyle{\pm 0.033}$ & $0.399 \scriptstyle{\pm 0.030}$\\
        
        & D-M  & $\mathbf{0.728 \scriptstyle{\pm 0.032}}$ & $\mathbf{0.492 \scriptstyle{\pm 0.060}}$ & $0.343 \scriptstyle{\pm 0.059}$ & $0.510 \scriptstyle{\pm 0.043}$ & $0.405 \scriptstyle{\pm 0.139}$\\
        & ED-M  & $0.713 \scriptstyle{\pm 0.008}$ & $0.483 \scriptstyle{\pm 0.031}$ & $\mathbf{0.395 \scriptstyle{\pm 0.035}}$ & $\mathbf{0.565 \scriptstyle{\pm 0.023}}$ & $\mathbf{0.603 \scriptstyle{\pm 0.017}}$
        \\
        
        % \midrule
        
        % BESO-Dec  & $0.742 \scriptstyle{\pm 0.103}$ & $0.503 \scriptstyle{\pm 0.035}$ &
        % \\
        % BESO-EncDec  & $0 \scriptstyle{\pm 0}$ & $0 \scriptstyle{\pm 0}$ &
        % \\
        
        % BESO-Mamba  & $0.808 \scriptstyle{\pm 0.038}$ & $0.580 \scriptstyle{\pm 0.051}$ &
        % \\
        % BESO-MambaDec  & $0 \scriptstyle{\pm 0}$ & $0 \scriptstyle{\pm 0}$ &
        % \\
        
	\midrule
        
\end{tabular}

}
\vskip -0.15in
\end{table}

==> results/tables/new_result_with_5history.tex <==
\begin{table}[hbtp]
\centering
\caption{Performance on LIBERO with 5 history}\label{main_results}
 
\resizebox{.95\textwidth}{!}{  

\begin{tabular}{l|c|ccc|cc}
	\toprule 

        \multicolumn{2}{c|}{history=5}  & \multicolumn{3}{c|}{w/o language} & \multicolumn{2}{c}{w/ language}\\

        \midrule
            
         Policy & Backbone & Libero-Object & Libero-Spatial & Libero-Long & Libero-Goal & Libero-90\\
        \midrule
        
        BC & D-T & $0.489 \scriptstyle{\pm 0.170}$ & $0.286 \scriptstyle{\pm 0.040}$ &$0.243 \scriptstyle{\pm 0.052}$ & $0.315 \scriptstyle{\pm 0.036}$ & $0.284 \scriptstyle{\pm 0.012}$
        \\
            & ED-T & $0.417 \scriptstyle{\pm 0.300}$ & $0.287 \scriptstyle{\pm 0.095}$ & $0.248 \scriptstyle{\pm 0.021}$ & $0.338 \scriptstyle{\pm 0.024}$ & $0.300 \scriptstyle{\pm 0.012}$
        \\
            & D-M & $\mathbf{0.765 \scriptstyle{\pm 0.115}}$ & $0.372 \scriptstyle{\pm 0.024}$ & $0.252 \scriptstyle{\pm 0.072}$ & $\mathbf{0.43 \scriptstyle{\pm 0.029}}$ & $0.529 \scriptstyle{\pm 0.094}$
        \\
            & ED-M & $0.743 \scriptstyle{\pm 0.020}$ & $\mathbf{0.428 \scriptstyle{\pm 0.029}}$ & $\mathbf{0.262 \scriptstyle{\pm 0.047}}$ & $0.317 \scriptstyle{\pm 0.105}$ & $\mathbf{0.599 \scriptstyle{\pm 0.019}}$ 
        \\
        
        \midrule
        
        DDP & D-T & $0.762 \scriptstyle{\pm 0.070}$ & $0.435 \scriptstyle{\pm 0.043}$ & $0.353 \scriptstyle{\pm 0.033}$ & $0.315 \scriptstyle{\pm 0.058}$ & $0.161 \scriptstyle{\pm 0.024}$
        \\
            & ED-T & $0.812 \scriptstyle{\pm 0.065}$ & $0.415 \scriptstyle{\pm 0.097}$ & $0.348 \scriptstyle{\pm 0.019}$ & $0.518 \scriptstyle{\pm 0.014}$ & $0.437 \scriptstyle{\pm 0.046}$
        \\
        
            & D-M & $\mathbf{0.815 \scriptstyle{\pm 0.004}}$ & $\mathbf{0.538 \scriptstyle{\pm 0.044}}$ & $0.387 \scriptstyle{\pm 0.040}$ & $0.388 \scriptstyle{\pm 0.027}$ & $0.352 \scriptstyle{\pm 0.096}$
        \\
            & ED-M & $0.778 \scriptstyle{\pm 0.005}$ & $0.513 \scriptstyle{\pm 0.024}$ & $\mathbf{0.417 \scriptstyle{\pm 0.023}}$ & $\mathbf{0.563 \scriptstyle{\pm 0.070}}$ & $\mathbf{0.455 \scriptstyle{\pm 0.081}}$
        \\
        
	\midrule
        
\end{tabular}

}
\vskip -0.15in
\end{table}

==> results/tables/num_data.tex <==
\begin{table}[hbtp]
\centering
\caption{Data Number ablation on LIBERO}\label{num_data}
 
\resizebox{.95\textwidth}{!}{  

\begin{tabular}{l|c|c|c|c}
	\toprule 

        History=5 & num\_data=5 & num\_data=10 & num\_data=30 & num\_data=50 \\

        \midrule
        
        BC-Dec  & $0.182 \scriptstyle{\pm 0.028}$ & $0.286 \scriptstyle{\pm 0.040}$ & $0.685 \scriptstyle{\pm 0.038}$ & $0.728 \scriptstyle{\pm 0.015}$ 
        \\
        BC-EncDec  & $0.147 \scriptstyle{\pm 0.114}$ & $0.287 \scriptstyle{\pm 0.095}$ & $0.578 \scriptstyle{\pm 0.096}$ & $0.732 \scriptstyle{\pm 0.016}$
        \\
        
        BC-Mamba  & $0.310 \scriptstyle{\pm 0.040}$ & $0.372 \scriptstyle{\pm 0.024}$ & $0.673 \scriptstyle{\pm 0.016}$ & $0.687 \scriptstyle{\pm 0.049}$ 
        \\
        BC-MambaDec  & $0.222 \scriptstyle{\pm 0.057}$ & $0.428 \scriptstyle{\pm 0.029}$ & $0.627 \scriptstyle{\pm 0.076}$ & $0.738 \scriptstyle{\pm 0.049}$
       
        \\
        
	\midrule

        History=1 & num\_data=5 & num\_data=10 & num\_data=30 & num\_data=50 \\

        \midrule
        
        BC-Dec  & $0.082 \scriptstyle{\pm 0.055}$ & $0.257 \scriptstyle{\pm 0.030}$ & $0.493 \scriptstyle{\pm 0.104}$ & $0.595 \scriptstyle{\pm 0.043}$ 
        \\
        BC-EncDec  & $0.122 \scriptstyle{\pm 0.010}$ & $0.333\scriptstyle{\pm 0.029}$ & $0.545 \scriptstyle{\pm 0.009}$ & $0.647 \scriptstyle{\pm 0.055}$
        \\
        
        BC-Mamba  & $0.278 \scriptstyle{\pm 0.070}$ & $0.410 \scriptstyle{\pm 0.058}$ & $0.657 \scriptstyle{\pm 0.043}$ & $0.685 \scriptstyle{\pm 0.072}$ 
        \\
        BC-MambaDec  & $0.237 \scriptstyle{\pm 0.106}$ & $0.352 \scriptstyle{\pm 0.069}$ & $0.567 \scriptstyle{\pm 0.075}$ & $0.627 \scriptstyle{\pm 0.024}$
       
        \\
        
	\midrule
        
\end{tabular}

}
\vskip -0.15in
\end{table}

==> results/tables/real_robot.tex <==
\begin{table}[hbtp]
\centering
\caption{Real Robot Experiement}\label{main_results}
 
\resizebox{.95\textwidth}{!}{  

\begin{tabular}{l|c|c|c}
	\toprule 

         history=5 & CupStacking & Inserting & Arranging \\

        \midrule
        
        DDPM-Dec  & $0.0 \scriptstyle{\pm 0.0}$ & $0.0 \scriptstyle{\pm 0.0}$ & $0.0 \scriptstyle{\pm 0.0}$ 
        \\
        DDPM-EncDec  & $0.0 \scriptstyle{\pm 0.0}$ & $0.0 \scriptstyle{\pm 0.0}$ & $0.0 \scriptstyle{\pm 0.0}$
        \\
        
        DDPM-Mamba  & $0.0 \scriptstyle{\pm 0.0}$ & $0.0 \scriptstyle{\pm 0.0}$ & $0.0 \scriptstyle{\pm 0.0}$
        \\
        DDPM-MambaDec  & $0.0 \scriptstyle{\pm 0.0}$ & $0.0 \scriptstyle{\pm 0.0}$ & $0.0 \scriptstyle{\pm 0.0}$
        \\
        
	\midrule
        
\end{tabular}

}
\vskip -0.15in
\end{table}

==> sections/mamba_agg.tex <==
\begin{algorithm}[H]
  \caption{ED-M DDP Inference} \label{alg:mamba_agg}
  \small
  \begin{algorithmic}[1]
    % \vspace{.04in}
    \Require Observation $\obs_{k-K:k}$, Mamba Encoder $\mathbf{Enc_m}$, Mamba Decoder $\mathbf{Dec_m}$, Position Embedding $\mathbf{PE}$, Learnable action variables $\hat{\act}_{k:k+J}$, learnable state variables $\hat{\obs}_{k-K:k}$, learnable time variables $\hat{t}$
    \State $\act^T_{k:k+J} \sim \mathcal{N}(\mathbf{0}, \textbf{I})$
    \For{$t=T, \dotsc, 1$}
      \State $E_t=\mathbf{Linear}(t)$
      \State $E_o=\mathbf{PE}(\mathbf{ResNet}(\obs_{k-K:k}))$
      \State $E_a=\mathbf{PE}(\mathbf{Linear}(\act^t_{k:k+J}))$
      \State $E_o=\mathbf{E_m}(cat(E_t, E_o, \hat{\act}_{k:k+J}))$ \Comment{Sequence alignment}
      \State $E_a=\mathbf{D_m}(cat(\hat{t}, \hat{\obs}_{k-K:k}, E_a)$ \Comment{Sequence alignment}
      \State $\act^{t-1}_{k:k+J}=\mathbf{D_m}(E_o+E_a)$ \Comment{Aggregation}
    \EndFor

    \State \textbf{return} $\act_{k:k+J}$
    % \vspace{.04in}
  \end{algorithmic}
\end{algorithm}

==> sections/method_depr.tex <==
\section{Method}
\label{sec:prelims}
\input{figures/architecture/architecture}
Diffusion policy with transformers has demonstrated great success in imitation learning. Compared to transformers, the newly introduced selective state space model, Mamba, achieves faster inference and state-of-the-art performance across different tasks such as language, image, etc.

\subsection{Mamba}
Recently, State Space Models (SSMs) have gained increased attention due to their effectiveness in various sequential tasks across language, audio, vision, and more. The Structured State-Space Sequence (S4) model, introduced by \cite{gu2021efficiently}, is emerging as a promising alternative to Transformers \cite{vaswani2017attention} for modeling sequential information. S4 model is inspired by a continuous system, $x(t) \in \mathbb{R} \mapsto y(t) \in \mathbb{R}$, that maps a 1-D input or sequence $x(t)$ into a hidden state $h(t) \in \mathbb{R}^\mathtt{N}$, which then can be projected into the output $y(t)$, 

\begin{equation}
\begin{aligned}
    h'(t) &= \mathbf{A}h(t)+\mathbf{B}x(t), \\ 
    y(t) &= \mathbf{C}h(t)
\end{aligned}
\end{equation}

where $\mathbf{A} \in \mathbb{R}^{\mathtt{N} \times \mathtt{N}}$ are the evolution parameters, $\mathbf{B} \in \mathbb{R}^{\mathtt{N} \times 1}$ and $\mathbf{C} \in \mathbb{R}^{1 \times \mathtt{N}}$ are the projection parameters. S4 transforms the parameters $(\mathbf{A}, \mathbf{B})$ to discrete parameters $(\mathbf{\overline{A}}, \mathbf{\overline{B}})$ through:

\begin{equation}
\begin{aligned}
\mathbf{\overline{A}} &= \exp{(\mathbf{\Delta}\mathbf{A})}, \\
\mathbf{\overline{B}} &= (\mathbf{\Delta} \mathbf{A})^{-1}(\exp{(\mathbf{\Delta} \mathbf{A})} - \mathbf{I}) \cdot \mathbf{\Delta} \mathbf{B}
\end{aligned}
\end{equation}

where $\mathbf{\Delta}$ is the step size. The model then can be computed using a linear recurrent way in Eq. (\ref{eq:discrete_lti})

\begin{equation}
\begin{aligned}
\label{eq:discrete_lti}
h_t &= \mathbf{\overline{A}}h_{t-1} + \mathbf{\overline{B}}x_{t}, \\
y_t &= \mathbf{C}h_t
\end{aligned}
\end{equation}

however, this recurrent computation cannot be parallelized. Therefore, SSM proposes to compute the output through a global convolution Eq. (\ref{eq:conv}).

\begin{equation}
\begin{aligned}
\label{eq:conv}
\mathbf{\overline{K}} &= (\mathbf{C}\mathbf{\overline{B}}, \mathbf{C}\mathbf{\overline{A}}\mathbf{\overline{B}}, \dots, \mathbf{C}\mathbf{\overline{A}}^{k}\mathbf{\overline{B}}), \\
\mathbf{y} &= \mathbf{x} * \mathbf{\overline{K}},
\end{aligned}
\end{equation}

Compared to the Transformer, which has an attention mechanism to select important elements, SSM does not provide a similar module to learn contextual information. Based on SSM, Mamba \cite{gu2023mamba} proposes a Selective Scan Operator to filter relevant features out and further design a hardware-aware algorithm to enhance computation efficiency. A comparison between self-attention and mamba block is visualized in Fig. \ref{}.

% Mamba is a new state space model architecture showing promising performance on information-dense data such as language modeling, where previous subquadratic models fall short of Transformers. It is based on the line of progress on structured state space models, with an efficient hardware-aware design and implementation in the spirit of FlashAttention.

\subsection{Diffusion Policies}

 
Based on DDPM and Mamba, we propose different architectures to incorporate Mamba in diffusion policy.

\subsection{Architecture}
% Put figures for different structures
We compare different designs for diffusion policy.
1. Decoder only transformer
2. Encoder-decoder transformer
3. Mamba only
4. Mamba cross


\subsection{Diffusion Mamba}
give an overview figure of the whole model
